Weakly-Supervised End-to-End CAD Retrieval to Scan Objects

CAD model retrieval to real-world scene observations has shown strong promise as a basis for 3D perception of objects and a clean, lightweight mesh-based scene representation; however, current approaches to retrieve CAD models to a query scan rely on expensive manual annotations of 1:1 associations of CAD-scan objects, which typically contain strong lower-level geometric differences. We thus propose a new weakly-supervised approach to retrieve semantically and structurally similar CAD models to a query 3D scanned scene without requiring any CAD-scan associations, and only object detection information as oriented bounding boxes. Our approach leverages a fully-differentiable top-$k$ retrieval layer, enabling end-to-end training guided by geometric and perceptual similarity of the top retrieved CAD models to the scan queries. We demonstrate that our weakly-supervised approach can outperform fully-supervised retrieval methods on challenging real-world ScanNet scans, and maintain robustness for unseen class categories, achieving significantly improved performance over fully-supervised state of the art in zero-shot CAD retrieval.

==> media/seen-transpose.tex <==
\begin{figure}[t]
  \centering
  \begin{tabular}{| c | c | c | c | c | c | c |}
    \hline
    Query & FPFH & PointNet & 3DCNN & JointEmb. & Ours & GT \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0000_02__12.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/53675c4bbb33fe72bcc0c5df96f9b28e.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/bfc242ae3d98762ece876412f61273f0.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/435ab5f43b24f739bc0c56c4d4a1fd3b.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/ab5c8c38528f06daf398d0c5832df00e.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/e7de8a24dfc385d92715de3ea7b582d7.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c904d927672acd48ad8a0ee9b106700e.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0439_00__0.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/68f1d9f63eae2b5123c1b1df1d480bd3.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/5b9b77ad6ce283a398e4bc44d45a32e.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/46de1dfe54a261b4c7e1f9c70054d66b.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/a06df01467d298caac51268fdb437a9e.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/4e89985989c6a1936aedbd2a02b96953.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/225905a8841620d7f6fe1e625c287cfa.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0253_00__0.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c55868566d2cd547d8d2db57c9e192a.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/e3f1f899d63ab008492d9da2668ec34c.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/40ab45735f526717e25492f5f62d416f.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/903a14845425ca3176e30bf48cd56fcd.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/1d0abb4d48b46e3f492d9da2668ec34c.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c8df724ce6f12ca2d86a257784298546.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0469_02__11.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/4848b62ac4a996b3f51f77a6d7299806.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/ab9e20f3f9d2f1d1d77c088a902d8fa1.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/45a4d128553abb329bf8498db368caef.jpg}
    \end{minipage}
     & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/cdf8eff26c940d7fcd1272091a2a216.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/45a4d128553abb329bf8498db368caef.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/4812245f2f9fa2c953ed9ce120377769.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0585_00__12.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/fa723633a3cfed271e74a5e93d408a1a.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/2a295b1bbb386e2f3ffa3a50996ad39e.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c2579f3b815ca02d9318709b609c3a71.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/48eecde6f71bc1a2f99d92708f91e592.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c2579f3b815ca02d9318709b609c3a71.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/9504267500abe76c510a6e7bd9c355b3.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0262_00__2.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/4d7ce41fe16725c5e346f79b9a86790.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/6d0cd48b18471a8bf1444eeb21e761c6.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/70eddfb0000447c637b2bb75885cfc44.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c0036465dcbeed6a912f115faa04d51.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/8769b3281dd41c771b17743c18fb63dc.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/f551048075b5042d7d6d37ceb4807b31.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0407_01__7.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/8c3c0ec3779a163098910e50f05b8001.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/227308a94bc7b231e5490ac94fb8e485.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/6df5ad89a152dbd26e79c14dd16aa04b.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c4e7fef0548b8d87247b7570b0fbe63d.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/c4e7fef0548b8d87247b7570b0fbe63d.jpg}
    \end{minipage}
     & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/97e2ca564decce0b575f9747ff6fb5e8.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0678_02__5.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/a52e8bd8b570f268f19146fa01c25917.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/9d62c46fc3fd343d1f9f3ce366e030fb.jpg}
    \end{minipage}
     & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/81be602470e4fa90b2f671e673cf292b.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/91b781b40d32b74dc491effd0ae881ea.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/226f73828ad8562f4c86b1fdc94892eb.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsizeje}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/5e411987081d3f3af44ef865a534c948.jpg}
    \end{minipage}
    \\ \hline
  \end{tabular}
\end{figure}

==> media/unseen-transpose.tex <==

\newcommand\imgsize{.16\textwidth}

\begin{figure}[!t]
  \centering
  \begin{tabular}{ | c | c | c | c | c | c | c |}
    \hline
    Scan & FPFH & PointNet & 3DCNN & JointEmb. & Ours & GT 
    \\ \hline
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0557_02__2.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/75dbeb01fdc7f265d0a96520c31993ad.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/2e149e4f08f7cbdfed4d676215f46734.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/f99f09473fa068dfc834d9ecc7d5f465.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/e083105e9c2a28bb0c3a03d0a1f182f.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/edf13191dacf07af42d7295fb0533ac0.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/e91c2df09de0d4b1ed4d676215f46734.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0024_00__19.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/e9a8bc335a7faf78f91663a74ccd2338.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/60f7d79d10e19134a3e7878f2bb5f0ca.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/7f523cf6780aaeda2a691a30a5c88605.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/28570547091748edc2cd59b38b35eb54.jpg}
    \end{minipage}
     & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/9a98a0088ac6d37a2c5b2f528cea9dd6.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/d8d129b1a07b23b7a738de48265832af.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0025_01__3.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/a97bd9998d12467d7275456565149f4f.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/21ee412299f40368df0c25a5c4f4cf31.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/9112f0ee6b1cdf5082ec48ff3a4fe07c.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/cb6e3dea697f87e55f0ba4cbc0133dcb.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/e58274d0771d56f77984fb9ec7e40829.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/abe41b86df0dcd5a3da04ac9f7df60de.jpg}
    \end{minipage}
    \\ \hline
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/scene0675_01__1.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/d0c3bf270f9e04eb362845c6edb57fc.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/4d81894947d08922beedb4c8fd29e2d1.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/506ce52bbfc7adecdb94e9396a25f7f1.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/40d0dd3fe786e120d75c27ddd792e41a.jpg}
    \end{minipage}
    & 
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/64c2347dfd79c63a63d977b06bbd429d.jpg}
    \end{minipage}
    &
    \begin{minipage}{\imgsize}
      \includegraphics[width=\linewidth]{media/Proxy Diagram/64c2347dfd79c63a63d977b06bbd429d.jpg}
    \end{minipage}
    \\ \hline
  \end{tabular}
\end{figure}
